Combining Global and Local Merges in Logic-based Entity Resolution

In the recently proposed Lace framework for collective entity resolution, logical rules and constraints are used to identify pairs of entity references (e.g. author or paper ids) that denote the same entity. This identification is global: all occurrences of those entity references (possibly across multiple database tuples) are deemed equal and can be merged. By contrast, a local form of merge is often more natural when identifying pairs of data values, e.g. some occurrences of 'J. Smith' may be equated with 'Joe Smith', while others should merge with 'Jane Smith'. This motivates us to extend Lace with local merges of values and explore the computational properties of the resulting formalism.

==> 5-Conclusion.tex <==
\section{Conclusion}\label{sec:Conclusion}

==> Comments.tex <==
1) I would suggest adding a sentence to this paper pointing to that discussion, or, better yet, pointing to the Appendix, which is extended with a discussion to related work, including newer work relevant to value merging.

Answer: Do we want to do this?

For a discussion of related work, see [Our PODS]. For omitted proofs, see [arXivVersion].

2) V is originally introduced at the bottom of page 1 as "the set V of value constants (or values)"; in Definition 3, on page 3, this changes to "equivalence relation V over Cells(D)". Easy to fix.

Answer: It is not the same symbol, the first one is in \mathsf. Do we want to use another symbol (e.g. \mathcal) to make them graphically even more different? 


3) - Please introduce
* the abbreviation DC
* the notation Cells() -- as used in Def.2
before using it.

Answer: I have introduced the abbreviation DC. The notation Cells has already been defined in the preliminaries.


4) Example 3: "that *it* is not possible"

Answer: Done


5) Theorem 2: wrong font for EqO and EqV

Answer: EqO and EqV are not mentioned in Th.2. Maybe the reviewer refers to Theorem 3, but in this case EqO and EqV are in the right font.


6) Gianluca: Do we want to mention most informative answers citing our IJCAI accepted paper?
